An Event Detection Approach Based On Twitter Hashtags

Twitter is one of the most popular microblogging services in the world. The great amount of information within Twitter makes it an important information channel for people to learn and share news. Twitter hashtag is an popular feature that can be viewed as human-labeled information which people use to identify the topic of a tweet. Many researchers have proposed event-detection approaches that can monitor Twitter data and determine whether special events, such as accidents, extreme weather, earthquakes, or crimes take place. Although many approaches use hashtags as one of their features, few of them explicitly focus on the effectiveness of using hashtags on event detection. In this study, we proposed an event detection approach that utilizes hashtags in tweets. We adopted the feature extraction used in STREAMCUBE and applied a clustering K-means approach to it. The experiments demonstrated that the K-means approach performed better than STREAMCUBE in the clustering results. A discussion on optimal K values for the K-means approach is also provided.

==> futurework.tex <==
\section{Future Work}

As with any study, some things could have been done better or more to further improve the results. The following are some recommendations for future research about this study.

\begin{itemize}
\item[--] Consider both spatial and temporal perspectives. In this study, we only considered the temporal perspective in the implementation and experiments. However, taking the spatial information into the implementation could make this study more practical for industry. For example, some events (e.g. local sport events) might not be discussed nationwide in lots of tweets but are densely discussed only in the tweets from certain areas. The characteristic could not be detected in our current approach. Considering both spatial and temporal perspectives could provide more information for event detection.
\item[--] Compare with more related works of hashtag clustering. Our original idea was to compare our method with \cite{feng2015streamcube}, \cite{middleton2014real}, and \cite{walther2013geo}. However, we only selected STREAMCUBE for some reasons: First, STREAMCUBE is the most relevant study to ours. Second, we could not find enough implementation details through the other two papers, and we were not able to reach the authors to use their original systems for our experiments. Although our approach was proved effective, a comprehensive comparison with the above different approaches could make our results more solid and convincing.
\item[--] Collect more manual labels from human subjects for the collected tweets. In this study, we only collected manual labels for 200 tweets that were randomly sampled from the collected tweets of November 17th, 2015. Because the number of our manual labels and human subjects are low, inviting more subjects and increasing manually labeled tweets could enhance the credibility of our experiments when comparing our approach to others.
\item[--] Analyze more events discussed on Twitter. We only collected the tweets related to the Paris Attack during November 13th to November 17th, 2015. Since this approach can be easily applied to any other events, it would be interesting if we could have applied our method on different datasets. If we could prove our approach also performs well on different datasets, it will demonstrate the practicality of this approach.
\item[--] Adopt other clustering approaches in our hashtag clustering module instead of K-means. Although we have shown K-means is effective in our study and could perform better than the clustering approach of STREAMCUBE, the best setting of K values may be varied in different datasets and is not easy to be determined. Even though we have discovered how to set K values in this study, it is still difficult to transfer the knowledge to other datasets. It is worth to adopt different clustering approaches that could self-adapt to different datasets in our hashtag clustering module. Moreover, adopting multiple different clustering approaches will show the extensibility of this study.

\end{itemize}
